Digraph Placement Games

This paper considers a natural ruleset for playing a partisan combinatorial game on a directed graph, which we call Digraph Placement. Given a digraph $G$ with a not necessarily proper $2$-coloring of $V(G)$, the Digraph Placement game played on $G$ by the players Left and Right, who play alternately, is defined as follows. On her turn, Left chooses a blue vertex which is deleted along with all of its out-neighbours. On his turn Right chooses a red vertex, which is deleted along with all of its out-neighbours. A player loses if on their turn they cannot move. We show constructively that Digraph Placement is a universal partisan ruleset; for all partisan combinatorial games $X$ there exists a Digraph Placement game, $G$, such that $G = X$. Digraph Placement and many other games including Nim, Poset Game, Col, Node Kayles, Domineering, and Arc Kayles are instances of a class of placement games that we call conflict placement games. We prove that $X$ is a conflict placement game if and only if it has the same literal form as a Digraph Placement game. A corollary of this is that deciding the winner of a Digraph Placement game is PSPACE-hard. Next, for a game value $X$ we prove bounds on the order of a smallest Digraph Placement game $G$ such that $G = X$.

==> my-symbols.tex <==
\makeatletter
\NewDocumentCommand{\fltrivb}{}{%
  <%
  \mathrel{%
    \mathpalette\scaled@parallel{r}%
  }%
}
\NewDocumentCommand{\fvbrtri}{}{%
  \mathrel{%
    \mathpalette\scaled@parallel{l}%
  }%
  >%
}
\newcommand{\scaled@parallel}[2]{%
  \if r#2\mkern-\scaled@parallel@kern{#1}mu\fi
  \vcenter{
    \m@th
    \sbox\z@{$#1<$}%
    \hbox{%
      \resizebox{\width}{\dimeval{\ht\z@+\dp\z@}}{%
        \raisebox{\depth}{$#1\parallel$}%
      }%
    }%
  }%
  \if l#2\mkern-\scaled@parallel@kern{#1}mu\fi
}
\newcommand{\scaled@parallel@kern}[1]{%
  \ifx#1\displaystyle 4.5\else
  \ifx#1\textstyle 4.5\else
  \ifx#1\scriptstyle 4.6\else
  5.1\fi\fi\fi
}
\makeatother
